Secure Calibration for Safety-Critical IoT: Traceability for Safety Resilience

Secure sensor calibration constitutes a foundational step that underpins operational safety in the Industrial Internet of Things. While much attention has been given to IoT security such as the use of TLS to secure sensed data, little thought has been given to securing the calibration infrastructure itself. Currently traceability is achieved via manual verification using paper-based datasheets which is both time consuming and insecure. For instance, when the calibration status of parent devices is revoked as mistakes or mischance is detected, calibrated devices are not updated until the next calibration cycle, leaving much of the calibration parameters invalid. Aside from error, any party within the calibration infrastructure can maliciously introduce errors since the current paper based system lacks authentication as well as non-repudiation. In this paper, we propose a novel resilient architecture for calibration infrastructure, where the calibration status of sensor elements can be verified on-the-fly to the root of trust preserving the properties of authentication and non-repudiation. We propose an implementation based on smart contracts on the Ethereum network. Our evaluation shows that Ethereum is likely to address the protection requirements of traceable measurements.

==> sections/deployment.tex <==
\section{Deployment}
\label{sec:deployment}

As the majority of blockchain solutions work best in a decentralised manner, doing so in this case allows for the collaboration between operators, manufacturers, regulators, and calibration agencies.

In the current state-of-the-art, calibration reports are stored centrally and any traceability-related operations require a manual inspection of such reports. While some trust blockchain technologies over larger, more established financial institutions, it is still the case that large fractions of the general population trust these institutions over blockchains. Thus, one of the key issues related to deploying our solution is trust, and if the public relies more on the current state-of-the-art than in our blockchain-based system, then this will be difficult to promote. However, the protection requirements that our solution envelops benefits the users of the blockchain data, providing anonymous reads and a source of reliable calibration data, to which the lower levels of trust may shift upward given some finite time post-deployment. Our solution solves the reintermediation problem, wherein the public using the blockchain would need to rely on a third-party for delegating interactions with the blockchain.

Unfortunately, the true boundary here is not purely situated at the user level, but rather at the organisational level. From the notions set out in our threat model and protection requirements, we chose to adopt a permissionless blockchain. The reason behind this is simple. Permissioned blockchains require prior approval from a central or delegated authority, which defeats the end goal of a decentralised collaborative system, as well as a need for identification to retrieve an address to interact with the data. Currently, many calibration organisations rely on the purchasing of read rights to calibration reports, excluding the owner(s) of the calibrated equipment, among other financial considerations. This may be a potential issue in proposing a decentralised collaboration between operators, manufacturers, calibration agencies, etc.

Furthermore, our proposed solution requires a digitised calibration report. Currently, there is no standard layout or set fields for data contained within calibration reports, and one issue that will arise is enforcement of standards across organisations and domains. For blockchain technologies in general, the lack of regulatory oversight is a disadvantage that pushes the adoption of such technologies away. The potential volatility of smaller agencies who may have the fear of missing out could be exploited by larger calibration agencies seeking this behaviour.

Overall, the case here is for security. The potential adoption relies on the users to understand the implications and inefficiency of the current state-of-the-art, and the benefits our solution provides, to set motion unto what seems an initially intimidating shift from current workflows, but is realistically a clear solution for a more secure, balanced and efficient calibration ecosystem.


==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

As we start to use connected devices to perform critical tasks, such as
performing surgical procedures on humans or other high assurance activities, ensuring that the
system can operate safely whilst being robust to attacks is
important. Additionally, we also require a strong tamper-resistant
trail of recorded activity to enable system forensics that will
withstand hostile scrutiny in a court of law. Indeed operational safety
breakdowns resulting in injury to humans working alongside connected
collaboration-robots (cobots) has  been the subject of much
litigation. These cases are illustrative of the significant
liabilities involved and the stakes involved in ensuring safety within
Industrial IoT settings. It is natural to pursue the development of
safety assurance system that can provide data traceability, support
decision forensics, and manage measurement uncertainty.

Our evaluation shows that the contract execution time for traceability
verification has a linear increase in cost with the number of
levels. Realistically though, the time required for contract execution
will depend on the dynamics of miner availability and competing
transactions. Further, the time required for the PoW scheme is two
orders of magnitude (tens to hundreds of seconds) larger than the
average verification time (a few hundred ms). As the most significant of all costs involved, mining time plays a crucial role given its variance. We note however,  that this is primarily due to the widely acknowledged inefficiency of the PoW scheme used currently by Ethereum. In due course, it is expected that other mainstream blockchain technologies will be available, that utilise other consensus approaches that enable scaling of the mining process and with higher efficiency. We have therefore computed the time consumed for contract execution, separate from mining and block confirmation times, with emphasis on contract execution. Based on our scalability tests it is clear that contract execution scales rather well, and the inefficiency of mining is a significant barrier to the frequency of on-the-fly calibration checks that an IoT device can afford.

\subsection{Limitations and Future Work}

\paragraphb{Parallelism:} The ethereum blockchain network was
conceived as a cryptographically secure and decentralized
database, with the capability to not only store data, but also execute
Turing complete code, allowing the network to function as a secure
virtual machine. The blockchain concept is merely a mechanism to
facilitate orderly updates to the data stored on the virtual machine
(so that there is no temporal ambiguity), and to ensure consensus
among all stakeholders. Each block is just a set of update calls
organised on the basis of their time of arrival to the processing node. And
since there is a possibility of dependence across certain transactions
which arrive one after another, all transactions must be processed
serially. Parallelism can only be incorporated across separate address
spaces, in which case transactions cannot directly access data stored
in different segments. The concept of sharding is based on this model
of splitting the database into independent chunks, and may be
incorporated into future blockchain networks. The current algorithm
requires modifications if it must benefit from sharding, because
currently, each entity (device/technician/organization) is logically
linked in the form of a tree.

\paragraphb{\# Supported devices:} The Ethereum network currently
prescribes that each block may only contain transactions whose total
gas cost amounts to 8 million at maximum. This is not only a result of
performance and financial considerations on the part of the nodes, but
the need to minimize the computation required by non nodes with low
computing power to validate blocks as well. As reported in the
evaluation, the gas cost of traceability-verification
(Write)~\ref{alg:getrootcert}, is around $200,000$ gwei per
execution. Thus assuming a (rather strict) regime of hourly
calibration verification, the cost is approx. 4 million gwei per
device. This means only 2 devices can be validated per block, assuming
that the system has access to the entire global bandwidth. Another
important consideration is the average block mining time. This was
rationalized not only based on monetary constraints, but also based on
studies conducted which measured the time taken for mined blocks to
propagate throughout a Blockchain network. Currently, the average
mining time for ethereum is around 15 seconds. This considerably
limits the number of fully harmonised traceability-verification
(write) requests to 11520 per day. As the total system bandwidth for
traceability-verification (write) is 11520 requests per day, this is a
key limitation that future work can focus on (There is no limit on
read-only traceability verification).

\paragraphb{Future work:} To decrease the gas cost (for write), we can
exploit the fact that our algorithm is built on a hierarchical model
of trust (which flows from the NMIs towards field devices). We can
leverage this to reduce the costs of traceability-writes. We can
introduce block {\em validators} -- trusted entities in our hierarchy
--- to validate blocks offline and write the correct result onto the
blockchain. Furthermore, a byzantinian fault tolerant (BFT) mechanism
can be incorporated among the block validators. This will ensure that
the write costs will be independent of the computational complexity of
Traceability Verification (Read only)~\ref{alg:getrootcert} algorithm,
while maintaining security.




% In comparison with the current state-of-the-art paper-based traceability verification, our protection mechanism not only provides a high level of integrity for ensuring complete chains, but also drastically minimises the time to verify a complete chain. The current state-of-the-art requires various steps at many different locations, relying on humans to process the request for each certificate and to manually check the certificate for the device's parents to continue.


==> solidity-highlighting.tex <==
% Copyright 2017 Sergei Tikhomirov, MIT License
% https://github.com/s-tikhomirov/solidity-latex-highlighting/

\usepackage{listings, xcolor}

\definecolor{verylightgray}{rgb}{.97,.97,.97}

\lstdefinelanguage{Solidity}{
	keywords=[1]{anonymous, assembly, assert, balance, break, call, callcode, case, catch, class, constant, continue, constructor, contract, debugger, default, delegatecall, delete, do, else, emit, event, experimental, export, external, false, finally, for, function, gas, if, implements, import, in, indexed, instanceof, interface, internal, is, length, library, log0, log1, log2, log3, log4, memory, modifier, new, payable, pragma, private, protected, public, pure, push, require, return, returns, revert, selfdestruct, send, solidity, storage, struct, suicide, super, switch, then, this, throw, transfer, true, try, typeof, using, value, view, while, with, addmod, ecrecover, keccak256, mulmod, ripemd160, sha256, sha3}, % generic keywords including crypto operations
	keywordstyle=[1]\color{blue}\bfseries,
	keywords=[2]{address, bool, byte, bytes, bytes1, bytes2, bytes3, bytes4, bytes5, bytes6, bytes7, bytes8, bytes9, bytes10, bytes11, bytes12, bytes13, bytes14, bytes15, bytes16, bytes17, bytes18, bytes19, bytes20, bytes21, bytes22, bytes23, bytes24, bytes25, bytes26, bytes27, bytes28, bytes29, bytes30, bytes31, bytes32, enum, int, int8, int16, int24, int32, int40, int48, int56, int64, int72, int80, int88, int96, int104, int112, int120, int128, int136, int144, int152, int160, int168, int176, int184, int192, int200, int208, int216, int224, int232, int240, int248, int256, mapping, string, uint, uint8, uint16, uint24, uint32, uint40, uint48, uint56, uint64, uint72, uint80, uint88, uint96, uint104, uint112, uint120, uint128, uint136, uint144, uint152, uint160, uint168, uint176, uint184, uint192, uint200, uint208, uint216, uint224, uint232, uint240, uint248, uint256, var, void, ether, finney, szabo, wei, days, hours, minutes, seconds, weeks, years},	% types; money and time units
	keywordstyle=[2]\color{teal}\bfseries,
	keywords=[3]{block, blockhash, coinbase, difficulty, gaslimit, number, timestamp, msg, data, gas, sender, sig, value, now, tx, gasprice, origin},	% environment variables
	keywordstyle=[3]\color{violet}\bfseries,
	identifierstyle=\color{black},
	sensitive=false,
	comment=[l]{//},
	morecomment=[s]{/*}{*/},
	commentstyle=\color{gray}\ttfamily,
	stringstyle=\color{red}\ttfamily,
	morestring=[b]',
	morestring=[b]"
}

\lstset{
	language=Solidity,
	backgroundcolor=\color{verylightgray},
	extendedchars=true,
	basicstyle=\footnotesize\ttfamily,
	showstringspaces=false,
	showspaces=false,
	numbers=left,
	numberstyle=\footnotesize,
	numbersep=9pt,
	tabsize=2,
	breaklines=true,
	showtabs=false,
	captionpos=b
}
